Aion: Better Late than Never in Event-Time Streams

Processing data streams in near real-time is an increasingly important task. In the case of event-timestamped data, the stream processing system must promptly handle late events that arrive after the corresponding window has been processed. To enable this late processing, the window state must be maintained for a long period of time. However, current systems maintain this state in memory, which either imposes a maximum period of tolerated lateness, or causes the system to degrade performance or even crash when the system memory runs out. In this paper, we propose AION, a comprehensive solution for handling late events in an efficient manner, implemented on top of Flink. In designing AION, we go beyond a naive solution that transfers state between memory and persistent storage on demand. In particular, we introduce a proactive caching scheme, where we leverage the semantics of stream processing to anticipate the need for bringing data to memory. Furthermore, we propose a predictive cleanup scheme to permanently discard window state based on the likelihood of receiving more late events, to prevent storage consumption from growing without bounds. Our evaluation shows that AION is capable of maintaining sustainable levels of memory utilization while still preserving high throughput, low latency, and low staleness.

==> sections/abstract-2.tex <==
% !TEX root = ../main.tex
Often enough, data streams of timestamped events can be susceptible to arbitrary large delays (e.g., network congestion). These delays can cause the events to be discarded in case they arrive after the corresponding window has been processed. Sidelining such events is not acceptable in mission-critical applications (e.g. money can be lost). However, modern Stream Processing Systems, that typically maintain window state entirely in memory, impose a tight limit on event lateness and/or degrade performance or even crash when memory runs out.

In this paper, we propose Aion, a comprehensive solution that
(i) offloads window state from memory to disk when computation is estimated to be far from happening;
(ii) uses a form of \emph{proactive caching}, where we take advantage of the semantics of stream processing computations to bring the data to memory ahead of the time when it is needed;
(iii) uses statistical inference to determine the appropriate amount of time to wait for all events pertaining to a window and purge the window state (Predictive Garbage Collection)
(iv) provides a customized trigger for past windows that is able to determine the execution times that minimize result staleness at a minimum amount of executions (necessary to comply with user-specified staleness bounds).

Experimental evaluation indicates that \name is capable of maintaining sustainable levels of memory utilization while still preserving high throughput, low latency, and low staleness.

==> sections/background-2.tex <==
% !TEX root = ../main.tex

% Streaming applications are commonly represented in the form of directed graphs that represent the \emph{data flow} of the application.
% The vertices of the graph are data transformations (operators), and its edges are channels that route data between operators.
% The data flowing along these edges is a stream, represented as a sequence of \emph{events}, each associated with a \emph{key} and a \emph{timestamp}.

An SPS reads data from one or more sources. The rate at which the data is read is called \emph{ingestion rate}. The rate at which an operator processes data is called \emph{processing rate}. For an SPS deployment to be sustainable, it requires  a processing rate able to  cope with the ingestion rate, at least on average over time.

\spara{Time domains.}
An important component of the abstraction provided by the operators is that events are associated with a timestamp. 
For assigning these timestamps, three different notions of time have been considered: \emph{processing-time}, \emph{ingestion-time}, and \emph{event-time}~\cite{Srivastava:2004:FTM:1055558.1055596}. With processing-time, each operator assigns a timestamp to an event based on the current system clock when it processes the event (difficult for replayability). Ingestion-time refers to the time when events enter the system, and is assigned to an event by the first operator that reads it from the data source. Finally, event-time is associated to an event at its origin (outside of the SPS) when it is generated. Event-time enables out-of-order streams of data events to be grouped and ordered by their timestamps, hence giving consistent results that are robust to delays (i.e., the result of the computation is the same irrespective of the order in which events are processed) or the mode of operation of the system~\cite{dataflow}. 

\spara{Windowing.}
A window groups events in time, allowing an infinite stream to be processed in finite batches~\citep{li2005semantics}.
A single event can be part of zero, one, or many windows, according to the user-specified semantics.
Common types of windows include: \textit{Tumbling}, fixed-size window with no overlap with other windows (e.g., to compute hourly aggregates); and \textit{Sliding}, fixed-size window that slides by some amount (e.g., compute hourly aggregates every 10 minutes).
% \textit{Session}: dynamically sized window, which represents a consecutive, data-dependent portion of the stream, usually defined per key (e.g., a group of events separated in time by no more than a defined gap constant); and \textit{Count}: window that groups a fixed number of consecutive events, irrespective of their timestamps.

\spara{Watermarks.}
When using event-time, a \emph{watermark} signals the time when the system {\em assumes} that all events up to a certain event timestamp $t$ have arrived at an operator~\citep{jefferson1985virtual}; e.g., a watermark can signal that (ideally) all events in a given window have been received.
However, events with a timestamp lower than the watermark timestamp $t$ may still be received, but are considered \emph{late}.
Late data may simply be dropped or, in case the SPS can handle lateness, incorporated into the state of a window that has already been processed.
In such a case, several semantics are possible, depending on the requirements of the application.
For instance, given an operator that computes the average of the values in a window, a late event might trigger the window to emit the new average incrementally by simply keeping track of the sum and the number of items, and updating these upon receiving late events. However, the case of non-linear functions such as percentiles or arbitrary UDFs is particularly complex: the whole state of the old window needs to be maintained in order to allow late events, and the whole computation needs to be re-executed.

There are two main types of watermarks: periodic and punctuated.
Periodic watermarks are emitted based on either processing time (every $p$ seconds) or stream elements (every $p$ events); whereas
punctuated watermarks are emitted based on conditions inferred from  data when a particular event arrives.
%For instance, a source might emit a watermark when an explicit flush event arrives.

% The generation of a watermark involves a delicate trade-off.
% If it is emitted in a conservative way, the system might wait longer than needed to process events, thus increasing latency.
% Conversely, if a watermark is premature, a large fraction of events will become late, thus adding overhead to the computation.
% Issuing watermarks is often based on a heuristic, since it is usually difficult to know when all events belonging to a window have arrived~\cite{murray2013naiad}.

\spara{Triggering.}
A trigger is a mechanism that determines when a windowed operation should be executed, i.e., when to compute the value of the function over the data in the window.
By default, a window is triggered when its watermark is emitted, but it can also be triggered at other times, using different policies, e.g., percentile based (when $50\%$ of the data has been accumulated), data based (counts, punctuation, pattern matching), or even via external signals. 
In addition, for late events, a window is also triggered when the system time has reached the watermark plus the \emph{maximum allowed lateness},  meaning  no further late events for the window are accepted, and the function value is final.

\spara{Operator State.}
Stateful operators must  maintain, typically in memory, events or information about them in order to perform aggregated computations (counts for aggregates, parts of the streams for pattern matching, model parameters for machine learning). Since there is no generally accepted API to maintain operator state, we focus, in this work, on the Flink state management API, through which operators can access a set of standard state prototypes. The first is \emph{ValueState}, where a single value can be maintained; e.g., a boolean indicating if an event key has been observed before in the current window. There is also \emph{ReducingState} and \emph{FoldingState}, where an operator maintains a single value that represents an aggregate of the processed substream, computed via a reduce or fold function; e.g., a per-key sum of events in the window. Finally, there is  \emph{ListState}, where an unbounded list of elements can be maintained (typically containing the accumulated events for the window).

\emph{ListState} is the most generic prototype,  used for custom operator functions. It is the most expensive in terms of memory, since this state grows monotonically with the number of received events. Each operator can declare several state elements, and Flink will manage their distribution and lifecycle (checkpointing and restoring). For each window processed by an operator, Flink maintains a separate instance of the operator state.

Flink default state backend  stores  entire state in memory. Thus,
when the maximum allowed lateness of an operator is large, the number of simultaneous windows can grow considerably, thus exerting high memory pressure. \name makes judicious use of persistent storage to limit memory utilization, thus alleviating this pressure, without sacrificing throughput or  latency.



==> sections/introduction.tex <==
% !TEX root = ../main.tex

%1) Mention the following(?): This problem can be solved by adding more machines. However, it will not be very resource efficiency to have machines whose memory is mostly occupied by inactive/late/past windows.
%2) Give more emphasis that handling late events it is important for security and accounting applications, maybe by giving one more example in addition to the ad impressions.

Processing large volumes of data in near real-time is becoming increasingly important in several application domains.
%such as identifying social network trends, characterizing advertisement campaign response, billing advertisers based on user engagement, detecting frauds and intrusions, system monitoring and diagnostics, and IoT applications, just to name a few.
Stream Processing Systems (SPSs)~\cite{bookstreams} are designed to address this need: they ingest streams of records and pass them through application-specific operators, which transform the stream and compute the final results.
Because of the increasing demand for real-time analytics over large flows of data, a number of distributed SPSs have been recently proposed, e.g., Storm~\cite{storm}, Spark Streaming~\cite{spark}, Samza~\cite{samza}, 
%(IBM Infosphere Streams, Microsoft StreamInsight, Streambase), 
Apex~\cite{apex}, Google Cloud Dataflow~\cite{googleclouddataflow}, and Flink~\cite{DBLP:journals/debu/CarboneKEMHT15}.
%Examples of streaming applications include identifying social network trends, characterizing advertisement campaign response, billing advertisers based on user engagement, detecting frauds and intrusions, and IoT applications, just to name a few.

% Event time processing, late messages are dropped
Most often, in streaming applications, each record in the stream represents a specific \emph{event} that is associated with an \emph{event time}, e.g., a user clicked on an ad at a certain time. Events are later processed by the SPS at a given \emph{processing time}, and events generated close in time are typically grouped into \emph{event time windows}, e.g., all clicks generated in the last hour.
%\todo{Say that late events inevitably arise in event-based systems because the window time for the aggregation does not necessarily coincide with the processing time at which events are made available to the system.}

The challenge with this model is that, invariably, some events will experience a large delay between when they are generated and when they are processed by the SPS.
%, i.e., the difference between their event time and processing time.
This delay can happen for a variety of reasons, e.g., due to communication delays, network failures, configuration errors, or the fact that the device that produced the event became temporarily unavailable or disconnected from the network before transmitting the event.
%As a consequence, stream processing systems must be able to handle \emph{late} events, i.e., events that arrive to the SPS too late to be included in the corresponding event time window.
%
Since waiting for events is at odds with providing near real-time results, modern SPSs return results quickly and refine them over time if needed.
While event time is not a new concept, this problem has not received much attention so far, as the systems and models that it affects are quite recent~\citep{dataflow}.

To illustrate this process, consider a dashboard that shows real-time trends in ad clicks.
The dashboard might group clicks in windows of a few seconds, and show aggregate metrics as soon as a window terminates.
After a window has been processed, the SPS stores it as a \emph{past window}.
Subsequently, any events that belong to this window in event time but that arrive after the window was processed are called \emph{late events}.
When a late event arrives, SPSs add them to the corresponding past windows, and process these windows again to produce up-to-date results.
In the ad click example, the dashboard will eventually be updated with all the late click events to provide accurate historical information. 

Handling late events with large delays is an important requirement in many applications. For example, Google's Photon system~\cite{Ananthanarayanan:2013:PFS:2463676.2465272}
%The application joins an ad impression stream with a stream of ad clicks generated at a close event time, for the purpose of billing advertisers.
%Joined data is arranged and aggregated in windows corresponding to the frequency with which advertisers are charged.
is used for ad billing, and the authors describe that, each time an ad click is permanently ignored due to delays, money is lost.  As a consequence, Google sets a very large threshold for ignoring late events (in the order of days), thus making such occurrence virtually impossible~\cite{Ananthanarayanan:2013:PFS:2463676.2465272}. Similarly, applications that log financial transactions may be forced to ensure that all events are incorporated in a given computation irrespectively of their arrival time, in order to meet accounting and legal constraints.

However, modern distributed SPSs are not equipped to handle late events with unbounded delays. They store past windows in memory, and consequently run out of memory very quickly, as we show in our evaluation.
The so-called ``lambda architecture''~\citep{marz2015big}, which requires to run a batch system alongside the SPS, is a solution to this problem.
However, it comes with the major downsides of requiring to operate and synch two different systems, two different codebases, and substantial delays in processing of the late events.
For these reasons, the lambda architecture has been abandoned in favor of systems such as Flink and Spark which are able to handle stream and batch processing on a single platform.

%Therefore, their threshold for ignoring late events is set to 3 days, which is beyond the capabilities of most current general-purpose SPS, since they need to store all events from this time period in memory, in order to recompute in case of the arrival of a late event.
%In the case of security or accounting applications, the implications of ignoring late events may be equally serious: important anomalous events might be missed, or financial transactions may not be recorded.

% If the streaming operator is a standard commutative and associative function, such as sum or average, aggregate window states are cheap to store and maintain incrementally. But streaming operators are often arbitrary User Defined Functions (UDFs) whose semantics are opaque to the SPS. Dealing with late events for these operators is challenging: updating speculative results based on late events requires re-executing the UDF over all events in the window, and therefore the window state must store all such events. Current SPSs store past windows in memory, and consequently applications with UDFs risk running out of memory very quickly, as we show in our evaluation.

In this paper, we propose \name, the first solution for a general-purpose SPS to be able to handle late events for the longest possible period, by making use of the full capacity that is available across primary and persistent storage (e.g., HDD, SSD, or NAS). 

A straightforward solution to this problem would be to bring data from secondary storage to memory on demand, whenever that data is needed as part of processing a late event. This is similar to the mechanism used by the OS to swap virtual memory (and may even rely on that implementation). However, as our evaluation shows, such on demand transfer of data between primary memory and persistent storage does not lead to adequate performance, due to the large performance gap between these storage levels, and because it generates too many concurrent random accesses. Conversely, when space in either primary or secondary storage is no longer available, the system must decide which events to evict, and today's general purpose heuristics such as LRU are not the best fit for SPSs.

To address this challenge, \name introduces two key techniques that leverage the semantics of stream processing in order to improve the management of data across memory and persistent storage.

The first technique is \caching, which treats main memory as a cache for the window state, which is otherwise offloaded to persistent storage.
The main insight of \caching is that the semantics of SPSs allow the system to predict that processing is more likely to be necessary at specific times, for example when a time window expires.
This enables using a {\em proactive} approach, where I/O is regulated by a central scheduler.
The scheduler leverages knowledge about the the timing of computations to proactively cache and evict ahead of time, thus minimizing the performance penalty of offloading to persistent storage in terms of both latency and throughput.
%The scheduler evicts the window state when memory pressure increases and computation is deemed far from happening. Conversely, it loads state from persistent storage to memory when computation is about to occur.

The second technique introduced by \name is \gc.
An SPS needs to eventually permanently delete past windows, when it is close to running out of persistent storage, but finding the right data to evict at the right time is difficult.
The system should guarantee that receiving late events for deleted past windows is extremely unlikely, but this depends on the distribution of inter-arrival times of the events, which depends on many deployment-specific factors and may be hard to predict a priori.
\gc uses the distribution of late event arrival to  predict inter-arrival times and thus to delete a window only when the likelihood of late events is under a user-specified threshold.

% Apart from these techniques, we also address the issue of updating late results. For past windows, it is desirable to amend previously emitted results as soon as late events arrive. However, recomputing a window (especially when associated with an UDF function) for each received event it is too computationally expensive. To address this, we provide a trigger that is able to find a good compromise between staleness of the result and resource usage (or number of executions), thereby identifying the adequate times for re-computing a past window.

To prove the effectiveness of our solution, we implemented \name by extending the codebase of Apache Flink, a widely-used distributed SPS; we are now in the process of trying to incorporate our modifications to the main codebase of Flink.
We extensively evaluate \name by using a number of benchmarks and practical applications.
Our results show that \name is able to handle late event with good performance, well beyond the limit where current SPSs run out of memory and crash. Furthermore, \name introduces a modest overhead when compared to the original system that keeps all state in memory.

%\todo{Highlight results here}.


%\subsection{Challenges}

%\begin{enumerate}
%	\item High Scalability. \mymark{unbounded lateness}
%	\item Low latency. \mymark{low overhead}
%   \item Processing rate. \mymark{should be competitive with baseline. I/O accesses need to be made efficient}
%    \item Transparency for applications. \mymark{applications should not be modified to work with our backend}
%\end{enumerate}


%\subsection{Contributions}
\if 0
The key contributions from this paper are:

\begin{enumerate}

%-- First to tackle the problem
\item We present \name, a window-management solution that enables SPSs to automatically maintain sustainable memory usage for unmodified long-lived streaming applications including arbitrary user-defined operators.

\item To achieve these goals we introduce two novel techniques, \caching and \gc, and a customized trigger that is able to minimize staleness of late executions at minimum expense.

\item We incorporate our techniques into the Apache Flink SPS.
Our source code is publicly available, and we are in the process of including \name in the main codebase of that framework.

\item We conduct an extensive evaluation using micro-benchmarks and realistic applications, and demonstrate the benefits of our approach.

\end{enumerate}
\fi

% roadmap
The remainder of the paper is organized as follows. Section~\ref{sect:background} provides the background and assumptions on stream processing necessary for later sections. Section~\ref{sect:architecture} presents our general architecture and design and implementation details. Section~\ref{sect:evaluation} presents our experimental evaluation. We survey related work in Section~\ref{sect:related-work} and conclude in Section~\ref{sect:conclusion}.
%Section~\S\ref{sect:evaluation}
%related work \S\ref{sect:related-work} 
%conclusion \S\ref{sect:conclusion} 
